Being a Bit Frequentist Improves Bayesian Neural Networks

Despite their compelling theoretical properties, Bayesian neural networks (BNNs) tend to perform worse than frequentist methods in classification-based uncertainty quantification (UQ) tasks such as out-of-distribution (OOD) detection. In this paper, based on empirical findings in prior works, we hypothesize that this issue is because even recent Bayesian methods have never considered OOD data in their training processes, even though this "OOD training" technique is an integral part of state-of-the-art frequentist UQ methods. To validate this, we treat OOD data as a first-class citizen in BNN training by exploring four different ways of incorporating OOD data into Bayesian inference. We show in extensive experiments that OOD-trained BNNs are competitive to recent frequentist baselines. This work thus provides strong baselines for future work in Bayesian UQ.

==> contents/91_derivations.tex <==
%!TEX root = ../main.tex


\subsection{The Dirichlet Log-Likelihood}
\label{subsec:app:dir_ll_derivation}

The $c$-dimensional Dirichlet distribution is a probability distribution over the $(c-1)$-probability-simplex. It has the log-density
%
\begin{align*}
    \log \mathrm{Dir}(y | \alpha) &:= \log \left( \prod_{c=1}^k (y^k)^{\alpha^k - 1} \frac{\Gamma \left( \sum_{k=1}^c \alpha^k \right)}{\prod_{k=1}^c \Gamma \left( \alpha^k \right)} \right) \\
        %
        &= \sum_{k=1}^c (\alpha^k - 1) \log y^k + \log \Gamma \left( \sum_{k=1}^c \alpha^k \right) - \sum_{k=1}^c \log \Gamma(\alpha^k) .
\end{align*}
%
Note that the superscript $k$ means the $k$-th vector component---not an exponent. Evaluated at the center of the simplex, i.e. at $\yout = (1/c, \dots, 1/c)$, we have
%
\begin{align*}
    \log \mathrm{Dir}(\yout | \alpha) &= -\sum_{k=1}^c (\alpha^k - 1) \log c + \log \Gamma \left( \sum_{k=1}^c \alpha^k \right) - \sum_{k=1}^c \log \Gamma(\alpha^k) \\
        %
        &= -\sum_{k=1}^c \alpha^k \log c - c \log c + \log \Gamma \left( \sum_{k=1}^c \alpha^k \right) - \sum_{k=1}^c \log \Gamma(\alpha^k) .
\end{align*}
%
Since we are only interested in making the softmax output of the network $F$ to be at the center of the simplex, we decouple $\alpha$ into its mean and precision terms \citep{minka2000estimating} and focus only on the mean, i.e. $\alpha = \gamma \mu$ with $\mu$ an element of the probability $(c-1)$-simplex and $\gamma = 1$. Furthermore, since we use this log-density function as a log-likelihood, we model the mean $\mu$ with the softmax output of $F$, i.e. $\mu = \sigma(F(\xout; \theta))$ for any OOD data $\xout \in \R^n$. Under this setup, the Dirichlet log-likelihood is given by
%
\begin{align*}
    \pout(\yout | \sigma(F(\xout; \theta))) &= -\sum_{k=1}^c \sigma(F(\xout; \theta))^k \log c + \log \Gamma \underbrace{\left( \sum_{k=1}^c \alpha^k \right)}_{= 1} - \sum_{k=1}^c \log \Gamma(\sigma(F(\xout; \theta))^k) + \mathrm{const} \\
        %
        &= -\sum_{k=1}^c \sigma(F(\xout; \theta))^k \log c - \sum_{k=1}^c \log \Gamma(\sigma(F(\xout; \theta))^k) + \mathrm{const} ,
\end{align*}
%
which is exactly the expression \eqref{eq:dir_ll}. Note that the log-gamma function required in this log-likelihood poses no problem implementation-wise since most deep learning libraries such as PyTorch and TensorFlow natively support this function.

